Robust Semantic Parsing with Adversarial Learning for Domain Generalization

This paper addresses the issue of generalization for Semantic Parsing in an adversarial framework. Building models that are more robust to inter-document variability is crucial for the integration of Semantic Parsing technologies in real applications. The underlying question throughout this study is whether adversarial learning can be used to train models on a higher level of abstraction in order to increase their robustness to lexical and stylistic variations.We propose to perform Semantic Parsing with a domain classification adversarial task without explicit knowledge of the domain. The strategy is first evaluated on a French corpus of encyclopedic documents, annotated with FrameNet, in an information retrieval perspective, then on PropBank Semantic Role Labeling task on the CoNLL-2005 benchmark. We show that adversarial learning increases all models generalization capabilities both on in and out-of-domain data.

==> motivation.tex <==
\section{Motivations}

Semantic Parsing models, such as Semantic Frame models, are used to extract events and scenarios (Frames) from a sentence, as well as semantic roles (Frame Elements) associated to them. One of the most popular semantic frame models is the Berkeley FrameNet  \cite{Baker:1998:BFP:980845.980860,fillmore2004framenet}.
Most works on Semantic Frame parsing follow a \textit{full text parsing} approach where all the lexical units (LU) from the FrameNet lexicon are considered potential \textit{frame triggers}. Annotating all the possible LU and frames in a sentence is a very difficult (and expensive) task for human annotators, therefore there are very few \textit{full text} annotations beyond the FrameNet 1.5 corpus. %Although the size of this benchmark is relatively large, a lot of frames have a very small number of occurrences in the corpus. This is due to the very large number of frames considered in the semantic model.

When processing domain specific corpora, the first baseline is to use a generic parser trained on FrameNet 1.5.  This corpus has been annotated using a \textit{full text parsing} scheme, allowing to perform comprehensive analysis of sentences. However, the drawback of this approach is that few examples are provided for each Frame and even though the senses from the FrameNet are generic, models trained on FrameNet 1.5 are not. Low performances due to poor generalization are a major issue in Frame semantic parsing \cite{nuges2009,sogaard2015using,hartmannout}. For this reason, using Frame Semantic parsers in downstream applications often requires to train new models on a corpus matching the applicative domains targeted. Assuming that such corpus will be available for each new domain or sub-domain to process is not realistic from an industrial perspective.

Part of the solution, given an applicative setting such as Information Extraction (IE) from specific domains where only a few frames related to IE targets are needed, is to adopt a \textit{partial  parsing} strategy, focusing on events and entities that are useful for the task. It is easier to put in place and large corpora can be manually annotated at a reasonable cost: the amount of frames and LU is limited and annotators can focus only on a few concepts.

% This is the scheme that was followed to annotate the CALOR Frame corpus~\cite{calor} used in this study which contains encyclopedic texts from several domains annotated with an IE perspective. The main differences between CALOR and FrameNet 1.5 is the limited size of the frame lexicon (only 103 frames) and the large amount of annotated examples for each frame in the corpus.
% Despite the feasibility of obtaining such partially annotated corpora, we can't expect, in a realistic setting, to always have a perfect match between training and application data. Domains can evolve, sub-domains can appear, and users expect a system not to break when processing a new document on a different but somehow related domain. In this context, developing semantic parsing models that are more robust toward stylistic or lexical variations is crucial from these approach to scale over realistic conditions. It is as well a challenging scientific issue for improving supervised learning methods.

% The goal of this study is to propose an adversarial setting for building domain-independent models that are more robust to document variability. This setting is applied in two conditions: when information about domains in the training corpus is known; and when no information is given prior to training. All settings are evaluated on an out-of-domain corpus showing that the adversarial scheme always improves system performance.

